Performance Impact of Memory Channels on Sparse and Irregular Algorithms

Graph processing is typically considered to be a memory-bound rather than compute-bound problem. One common line of thought is that more available memory bandwidth corresponds to better graph processing performance. However, in this work we demonstrate that the key factor in the utilization of the memory system for graph algorithms is not necessarily the raw bandwidth or even the latency of memory requests. Instead, we show that performance is proportional to the number of memory channels available to handle small data transfers with limited spatial locality. Using several widely used graph frameworks, including Gunrock (on the GPU) and GAPBS \& Ligra (for CPUs), we evaluate key graph analytics kernels using two unique memory hierarchies, DDR-based and HBM/MCDRAM. Our results show that the differences in the peak bandwidths of several Pascal-generation GPU memory subsystems aren't reflected in the performance of various analytics. Furthermore, our experiments on CPU and Xeon Phi systems demonstrate that the number of memory channels utilized can be a decisive factor in performance across several different applications. For CPU systems with smaller thread counts, the memory channels can be underutilized while systems with high thread counts can oversaturate the memory subsystem, which leads to limited performance. Finally, we model the potential performance improvements of adding more memory channels with narrower access widths than are found in current platforms, and we analyze performance trade-offs for the two most prominent types of memory accesses found in graph algorithms, streaming and random accesses.

==> experimental-setup.tex <==
% \newcommand{\rowspace}{\hspace{0pt}}
% \newcommand{\colspace}{\hspace{0pt}}
% %\newcommand{\fline}[1]{\multicolumn{1}{c}{\textbf{#1}}}
% \newcommand{\fline}[1]{\multirow{2}{*}{\textbf{#1}}}
% \colorlet{lgrey}{black!6}

\input{experimental-tables}


% To test the impact of the memory channelsGunrock \cite{wang2017gunrock} on the performance of graph algorithms, we ran multiple benchmarks on both CPU and GPU systems. The exact benchmarks are discussed below and are different for these unique architectures. For example, on the GPU systems the memory configuration is predefined and is part of the actual processor. For the CPU, we are able to control the number of channels based on the number of DIMMs used as well as their placement on the motherboard.

The graphs used in the experiments are taken from SNAP \cite{Snap-Stanford} and the Florida Matrix Market \cite{florida-matrix} repositories, with details to be found in Table \ref{tab:graphs}. All edges as treated as undirected. Also, all self-loops, duplicate edges, and singleton vertices are removed in a preprocessing phase. Lastly, vertex IDs were randomized and the graphs relabeled to increased random memory access patterns (some of these graphs had been previously relabeled to improve locality). 
% Such relabeling could have significant impact on performance (cite?) but it outside the scope of this paper. 



\vspace{-0.15cm}
\subsection{GPU Setup}

To measure the impact of the memory channels on the performance of graphs on the GPUs we use the highly optimized Gunrock \cite{wang2017gunrock} library. We also use algorithms from \NVG, a linear-algebra based graph analytics library by NVIDIA. These experiments were conducted on four different NVIDIA Pascal-generation GPUs (details in Table \ref{tab:gpu-cpu-systems}). While the GPUs differ in cores counts and clock frequencies, these are not substantial. The biggest difference between them in core count is 7\% and clock speed is 26\%. The P100 also has a larger L2 cache size (4 MB) compared to the others (3 MB). While this has some impact on smaller inputs, larger networks are orders of magnitude larger than L2 size, meaning the majority of accesses should reach main memory. Therefore we focus on the GPUs' memory subsystems as their biggest distinction. Note the difference in the available bandwidth on these systems from the lowest bandwidth of 345 GB/s on the P40 to the highest bandwidth of  720 GB/s on the P100. %However, the bandwidth is not entirely indicative of the performance of the graph algorithms. 


\vspace{-0.1cm}






==> model-backup.tex <==

In the two previous experimental system we took an in-depth at the behavior of several widely used graph algorithms. Contrary to the past sections which looked at the algorithm as a whole, in this section we take an indepth look at the behavior of the algorithm and distinguish between two types of very different memory accesses. These memory accesses are typically encountered in sparse problems: random memory access and consecutive memory accesses.

\begin{algorithm}[t]

\scriptsize

    
    \For {$v \in V$}
    {
        $PR_{curr}[v] \leftarrow 0$ \\
        $C[v] \leftarrow Pr_{prev}[v]/deg[v]$
    }

    \For {$v \in V$}
    {
    // ``Streaming edge'' access\\
        \For {$v \in Neighbors[u]$} 
        {
	        // Random access \\
        	$PR_{curr}[v] \leftarrow PR_{curr}[v] + C[u] $ 
        }
    }
    \For {$v \in V$}
    {
        $PR_{curr}[v] \leftarrow \frac{1-d}{NV} + d\cdot PR_{curr}[v]$\\
        $PR_{prev}[v] \leftarrow Pr_{curr}$
    }


\caption{Page-Rank pseudo code.}
\label{alg:pr}

\end{algorithm}





Specifically, for this case study we select the widely used Page Rank analytic which ranks vertices based on the number of random walks that go through each vertex.  
Numerous algorithms have been designed for Page Rank, including sharding based algorithms  \cite{kyrola2012graphchi,cusha,zhou2017design}, gather-apply-scatter \cite{beamer2017reducing}, and linear algebra \cite{}. 
For the sake of simplicity we use a very simple Page Rank, Alg. \ref{alg:pr} for our analysis. Our reasons are two fold. First of all, all the aforementioned algorithms have the same two key types of memory accesses even if these are implemented differently due to the different programming models. Second, several of these algorithms, such as \cite{zhou2017design,beamer2017reducing}, have been designed to reduce the number of random memory accesses. In most cases, these algorithm end up being more efficient, yet they also do not stress the memory system. Furthermore, these algorithms were designed to optimize a specific problem. Our use of Page Rank is to highlight a problem that exists in various types of graph algorithms.


In the upcoming experiments, we use and modify the PageRank implementation from Ligra. Our variation is entirely pull-based. For simplicity, we fix the number of PageRank iterations at 20. We have also update the Ligra implementation to us an $O(|V|)$ division operations instead of $O(|E|)$ - this removes computational overheads from our analysis. Additional modifications were made to Ligra to enable our emulation of the narrow memory channels.
Performance is evaluated on for the $liveJournal$ graph and is executed on the KNL server described earlier in this paper. 

% We furthermore modify the code for \textit{streaming} and \textit{adjacency gap}. For the adjacency gap experiments, we've preprocessed out a division operation that accompanies every edge update. 


\subsection{Memory Access Types}

In this work we differentiate between two main types of memory access. We refer to the first type of access as ``{\bf graph streaming}'. These accesses focus on fetching in elements of the graph, such as vertices or edges (usually in the format of an adjacency list). In the case of Page Rank, these access can be thought of as traversing the neighbors of a given vertex. Note that the adjacency array can be in consecutive memory if the right data structure is used, as is the case for CSR or a sorted edge list.
The second type of memory access refers to ``{\bf random memory}'' accesses which are usually used by the analytic itself to update and store specific values. For Page Rank, these are the PR values, for BFS these can be the distances for the root, and for matching algorithms these can be scores of a vertex or edge. The sequence of these accesses is typically driven by the input and a previous set of events. Further, these accesses can be all over the memory space used by the analytic - making them {\bf random} by nature. In the context of PageRank, for each traversed neighbor, a ranking value is fetched for each traversed neighbors. Given that the neighbors of a vertex might not be in a consecutive space these require random memory accesses. Now note the following, the number of random memory access is on roughly the same order of magnitude as those of the graph streaming accesses; after all, each random memory access is dependent on edge that was streamed in. This is an important observation for the narrow memory channel analysis.




\begin{figure}[t]
\centering
  \includegraphics[width=\columnwidth]{figures/ligra-PR-memory-figures/cilk-dram-pcm-streaming_normalized.pdf}

  \caption{Adjacency traversal-only execution time as ratio of overall PageRank execution time for DDR memory.}

\label{fig:streaming}	


Fig. \ref{streaming} depicts the percentage of time spent streaming in the graph out of the total execution time for the DDR memory \footnote{In practice, this phase includes the entire page rank computation except for the random memory accesses.}. The abscissa depicts the number of threads used for each experiment. While there is a slight difference between the percentage across the threads, the overall time spent in this phase is relatively small in comparison to the time spent in the random access part. This is not overly surprising as traversing the adjacency array benefits for cache re-usability. Further, these streaming accesses also benefit from prefetching. 




\end{figure}

\begin{figure}[t]
\centering
 \includegraphics[width=0.9\columnwidth]{figures/ligra-PR-memory-figures/cilk-dram-pcm-bandwidth.pdf}

  \caption{Bandwidth for PageRank execution (streaming and random memory accesses) for the DDR memory . Measured using \textit{Intel PCM}.}

\label{fig:bandwidth-dram}	

\end{figure}



\begin{figure}[t]
\centering
 \includegraphics[width=0.9\columnwidth]{figures/ligra-PR-memory-figures/cilk-vtune-l2misses.pdf}

  \caption{Total L2 (LLC) misses measured by \textit{Intel VTune}. Counts are nearly identical using either DRAM or MCDRAM numa preference, which is expected.}

\label{fig:l2-misses}	

\end{figure}






\subsection{Narrower Channels}

Given the above discussion on the performance of the different memory accesses, we attempt to analyze the behavior of PageRank given a narrower memory channel. For most random memory accesses, whenever a cache line is fetched in only a single data element is used. As such, a narrower memory channel which brings only the necessary data is not likely to reduce the performance of these accesses.
Consider a cache line of 64 bytes with 4 bytes memory accesses. Given that a random memory access will bring in a whole cache line and we only use 4 bytes of that data, the utilization of that cache line is $6.25\%$. 
While, an additional element of that cache line might be used, in practice the data reuse is fairly small.
Therefore, reducing the width of the channel to bring will greatly increase the utilization of the fetched data. From a power perspective, by bringing in only the necessary data, it is actually possible to reduce the overall power consumption of the system.

As such, we attempt to understand how the narrower channels will affect the edge streaming phase.
For the graph streaming phase, the analysis is quite different. Recall that an adjacency array is usually in a consecutive place in memory. This means that in current systems, when fetching an adjacency array into the cache, it is very likely that multiple edges will fall into a single cache line. This allows for overall good usage of fetched data. For large adjacency arrays, the system can also pre-fetch data allowing for better system utilization. For smaller adjacency arrays, the data reuse might be lower. Yet, this does not seem to be a major problem according to  Fig. \ref{fig:streaming}. In fact, narrow channels could lead to better data reuse for the smaller vertices. In all likelihood, it is the bigger vertices that would probably be affected by the narrower channels as the number of memory requests to bring in the adjacency array will increase. The job of the prefetcher might prove to be more challenging.


% Given the results shown earlier in this paper, it would seem that adding additional memory controllers and channels into the memory sub-system would help alleviate some of the stress for large thread counts. Such an answer is of course contentious as adding more channels could result also in increasing the number of lanes between the CPU and the memory; this could increase power consumption as well as increase costs to the motherboard as well as the processor. Instead, we try to resolve in this a more friendly manner and attempt to use a framework as close to the ones that are currently manufactured. 

% Specifically, we speculate on the performance of sparse and irregular algorithms under the assumption that current channels are divided into a larger number of narrower sub-channels\footnote{In fact each of these sub-channels would be its own separate entity and would work like a regular. We use this the term {\bf sub-channel} to highlight the difference between current technology and the speculated memory sub-system.}. By decreasing the channel width by the same factor that the number of channels is increased, we effectively maintain the overall bandwidth of the system
% Note, the following analysis does not show to actually design such a system, rather it shows the pros and cons of such an approach. 




\subsection{Narrower Sub-Channel Emulation}  

TODO: cite section that discusses memory widths

Earlier in this paper, Section \ref{sec:memory}, we discussed the parameters of the different memory sub-systems. From a user's perspective, these parameters are invariant and non-configurable. 
As such, a memory channel cannot be divided into narrower sub-channels to test the above hypothesis in hardware. Instead, we design a software experiment that gives a first order approximation of having a narrower channel.
The experiments works as follows, given an adjacency array $[x,y,z]$ we insert dummy values, $\bullet$, into the adjacency arrays such that the new adjacency is $[x,\bullet^1,\bullet^2,...,\bullet^k,y,\bullet^1,\bullet^2,...,\bullet^k,z,\bullet^1,\bullet^2,...,\bullet^k]$, where $k$ refers to the number of dummy values inserted between to edges in the original input. These dummy values are ignored in the execution of the algorithm \footnote{Our modified implementations jumps over the dummy values without accessing them.}. 
We refer to $k$ as the {\bf gap} size. By using a gap great than one ($k>=1$), we increase the stress on the memory sub-system. For example, adding a single dummy value will require fetching in twice the number of cache lines than required if no dummy values are added. For $k=3$, the number of cache misses will be four times as high. While the utilization of the fetched data goes down with the increase of $k$, we are able to emulate the behavior of a narrower channel (albeit we only have one narrower channel instead of multiple channels). Given channels of width 64 bytes and using 4 bytes to represent an index, using a gap of $k=15$, we ensure that only a single value of each cache line is used.  


Fig. \ref{fig:gap-streaming} and Fig. \ref{fig:gap-total} depict the execution time of the graph streaming phase and the total execution time, respectively. The abscissa represents the gap size. Gap size of $k=0$ represents the results for the original input graph without any dummy values inserted into the graph.
We show the execution time for multiple thread counts for both the DDR memory as well as the MCDRAM. 
For the DDR based memory, it is quite clear that increasing the GAP increases the execution time. For 16 threads, this becomes visible at gap $k=4$. For the larger thread counts it is already apparent at $k=4$ where the execution increase by over $50\%$.

\begin{figure*}[t]
\centering
\subfloat[DRAM]{
 \includegraphics[width=0.9\columnwidth]{figures/ligra-PR-memory-figures/cilk-dram-adjacencyGap-times_streaming.pdf}}
\subfloat[MCDRAM]{
 \includegraphics[width=0.9\columnwidth]{figures/ligra-PR-memory-figures/cilk-hbm-adjacencyGap-times_streaming.pdf}}

  \caption{Increasing gap size (powers of 2) vs. execution time for only the edge-traversal phases of Ligra PageRank. Comparison is between using DRAM and MCDRAM memory on the KNL. Gap size of 16 onwards emulates cache line accesses with no data reuse. }

\label{fig:gap-streaming}	

\end{figure*}


\begin{figure*}[t]
\centering
\subfloat[DRAM]{
 \includegraphics[width=0.9\columnwidth]{figures/ligra-PR-memory-figures/cilk-dram-adjacencyGap-times.pdf}}
\subfloat[MCDRAM]{
 \includegraphics[width=0.9\columnwidth]{figures/ligra-PR-memory-figures/cilk-hbm-adjacencyGap-times.pdf}}

  \caption{Increasing gap size (powers of 2) as a function of the overall execution time for Ligra PageRank for different thread counts (16, 64, or 256): (a) DDR and (b) MCDRAM. Gap size of 16 onwards emulates a single cache line access with no data reuse. }

\label{fig:gap-total}	

\end{figure*}



\begin{figure*}[t]
\centering
\subfloat[DRAM]{
 \includegraphics[width=\columnwidth]{figures/ligra-PR-memory-figures/cilk-dram-adjacencyGap-times_scatter.pdf}}
\subfloat[MCDRAM]{
 \includegraphics[width=\columnwidth]{figures/ligra-PR-memory-figures/cilk-hbm-adjacencyGap-times_scatter.pdf}}

  \caption{Number of threads used as a function of overall execution time for Ligra PageRank. The different curves represent performance scaling for different gaps introduced into the graph. The two plots compare using DRAM and MCDRAM memory for the same experiments.}

\label{fig:gap-scaling}	

\end{figure*}


\begin{figure}[t]
\centering
 \includegraphics[width=0.9\columnwidth]{figures/ligra-PR-memory-figures/cilk-dram-adjacencyGap-streaming_normalized.pdf}


  \caption{Edge streaming normalized to total time, for different adjacency gap sizes (DRAM-only).}

\label{fig:normalized-dram}	

\end{figure}



\begin{figure}[t]
\centering
 \includegraphics[width=0.9\columnwidth]{figures/ligra-PR-memory-figures/cilk-hbm-adjacencyGap-streaming_normalized.pdf}


  \caption{Edge streaming normalized to total time, for different adjacency gap sizes (MCDRAM-only)}

\label{fig:normalized-mcdram}	

\end{figure}



\begin{figure}[t]
\centering
 \includegraphics[width=0.9\columnwidth]{figures/ligra-PR-memory-figures/cilk-dram-adjacencyGap-bandwidth.pdf}


  \caption{}

\label{fig:bandwidth}	

\end{figure}








%%%%%%% Before modifications

% \subsection{Algorithm and Memory Sub-system Co-Design }

% In this section we attempt to tackle an important question: ``What new architectural features are needed for the memory subsystem in order for it to be efficient for sparse and irregular applications?''.  Given the results shown earlier in this paper, it would seem that adding additional memory controllers and channels into the memory sub-system would help alleviate some of the stress for large thread counts. Such an answer is of course contentious as adding more channels could result also in increasing the number of lanes between the CPU and the memory; this could increase power consumption as well as increase costs to the motherboard as well as the processor. Instead, we try to resolve in this a more friendly manner and attempt to use a framework as close to the ones that are currently manufactured. 
% Specifically, we speculate on the performance of sparse and irregular algorithms under the assumption that current channels are divided into a larger number of narrower sub-channels\footnote{In fact each of these sub-channels would be its own separate entity and would work like a regular. We use this the term {\bf sub-channel} to highlight the difference between current technology and the speculated memory sub-system.}. By decreasing the channel width by the same factor that the number of channels is increased, we effectively maintain the overall bandwidth of the system
% Note, the following analysis does not show to actually design such a system, rather it shows the pros and cons of such an approach. 

% TODO: Do we have an proof or a citation to a paper that shows that the amount of data used in each random memory access is small?

% As a first step in this process, we consider the impact of a narrower impact on the performance of the two aforementioned memory accesses. We start off with the random memory accesses. These accesses would not be affected by the reduction in the width of the channel as in most cases as only a small part of the cache line is used for each fetched element. Consider a cache line of 64 bytes with 4 bytes memory accesses. Given that a random memory access will bring in a whole cache line and we only use 4 bytes of that data, the utilization of that cache line is $6.25\%$. While, an additional element of that cache line might be used, in practice the data reuse is fairly small within a single cache line. As such, reducing the width of the channel to bring in smaller elements will not affect re-usage however will greatly increase the utilization of the data that was fetched. From a power perspective, by bringing in only the necessary data, it is actually possible to reduce the overall power consumption of the system.

% For the graph streaming phase, the analysis is quite different. Recall that an adjacency array is usually in a consecutive place in memory. This means that in current systems, when fetching an adjacency array into the cache, it is very likely that multiple edges will fall into a single cache line. This allows for overall good usage of fetched data. For large adjacency arrays, the system can also pre-fetch data allowing for better system utilization. For smaller adjacency arrays, the data reuse might be lower. Yet, this does not seem to be a major problem according to  Fig. \ref{fig:streaming}. In fact, narrow sub-channels would lead to better data reuse for the smaller vertices. It is the bigger vertices that would probably be affected by the narrower sub-channels as the number of memory requests to bring in the adjacency array will increase. Further, the job of the prefetcher might prove to be more challenging though current pre-fetching techniques might also be viable options.

% \subsection{Narrower Sub-Channel Emulation}  

% TODO: cite section that discusses memory widths

% Earlier in this paper we discussed the parameters of the different memory sub-systems. From a user's perspective, these parameters are invariant and non-configurable. As such, a memory channel cannot be divided into narrower sub-channels to test the above hypothesis in hardware. Instead, we design a software experiment that gives a first order approximation of having a narrower sub-channel. The experiments works as follows, given an adjacency array $[x,y,z]$ we insert dummy values, $\bullet$, into the adjacency arrays such that the new adjacency is $[x,\bullet^1,\bullet^2,...,\bullet^k,y,\bullet^1,\bullet^2,...,\bullet^k,z,\bullet^1,\bullet^2,...,\bullet^k]$, where $k$ refers to the number of dummy values inserted between to edges in the original input. These dummy values are ignored in the execution of the algorithm. 
% We refer to $k$ as the {\bf gap} size. While using a gap great than one ($k>=1$), we increase the stress on the memory sub-system. For example, adding a single dummy value will require fetching in twice the number of cache lines than required if no dummy values are added. For $k=3$, the number of cache misses will be four times as high. While the utilization of the fetched data goes down with the increase of $k$, we are able to emulate the behavior of a narrower channel (albeit we only have one narrower channel instead of multiple channels). Given channels of width 64 bytes and using 4 bytes to represent an index, using a gap of $k=15$, we ensure that only a single value of each cache line is used.  


% TODO: is the gap size in the plots the actual gap size or is it the size of the new edge?

% Fig. \ref{fig:gap-streaming} and Fig. \ref{fig:gap-total} depict the execution time of the graph streaming phase and the total execution time, respectively. The abscissa represents the gap size. Gap size of $k=0$ depicts the results for the original input graph without any dummy values inserted into the graph.
% We show the execution time for multiple thread counts for both the DDR memory as well as the MCDRAM. 
% For the DDR based memory, it is quite clear that increasing the GAP increases the execution time. For 16 threads, this becomes visible at gap $k=4$. For the larger thread counts it is already apparent at $k=3$ where the execution increase by over $50\%$.
